Self-supervised Transparent Liquid Segmentation for Robotic Pouring

Liquid state estimation is important for robotics tasks such as pouring; however, estimating the state of transparent liquids is a challenging problem. We propose a novel segmentation pipeline that can segment transparent liquids such as water from a static, RGB image without requiring any manual annotations or heating of the liquid for training. Instead, we use a generative model that is capable of translating images of colored liquids into synthetically generated transparent liquid images, trained only on an unpaired dataset of colored and transparent liquid images. Segmentation labels of colored liquids are obtained automatically using background subtraction. Our experiments show that we are able to accurately predict a segmentation mask for transparent liquids without requiring any manual annotations. We demonstrate the utility of transparent liquid segmentation in a robotic pouring task that controls pouring by perceiving the liquid height in a transparent cup. Accompanying video and supplementary materials can be found

==> 5-results-old.tex <==
\section{RESULTS}

\subsection{Dataset Description}

To train our method, 
%we collected two raw RGB datasets $\mathcal{I}_{\mathrm{color}}, \mathcal{I}_{\mathrm{transparent}}$ using the procedure outlined in Section \ref{sec:dataset_collection}. We 
%we selected a static scene from our lab space, 
we collected 4 distinct pouring videos each of green-colored water and clear water. This resulted in datasets with 2231 and 2237 RGB frames, respectively. We also collected a test set of 133 images of transparent liquids in the same scene.
%, with roughly $\frac{1}{3}$ comprising images of an empty cup, $\frac{1}{3}$ of dynamic pouring, and $\frac{1}{3}$ of settling/still liquid levels. \ben{more exact numbers, maybe}

% Describe the dataset we collected (i.e. environment). Maybe this is the time to include the TV?

% \dave{I assume by ``TV" you mean using a video to learn to be invariant to different backgrounds. wouldn't put it here since the ``TV" was not used in all experiments. I would either: 1) Describe it in the last part of the methods section, and then clearly describe which experiments we use it for, or 2) Describe it in a separate methods subsection where you talk about the background invariance}

\subsection{Segmentation performance}

To evaluate the segmentation performance of the method for transparent liquids, we create a test set of 133 images of transparent containers that have varying amounts of transparent liquids (water) in them, placed at different distances from the camera.  We manually annotate the location of the transparent liquids for the test set using \cite{labelme};  however, we do not use such annotations for training. 

\begin{table}[ht]
    \centering
    \begin{tabular}{|c|c|c|c||c|}
        \hline
        Method & Low & Medium & High & All \\ 
        \hline
         Ours & 0.56 & 0.78 & 0.84 & 0.72  \\
         \hline
         Supervised (10\%) & 0.61 & 0.91 & 0.86 & 0.79  \\
         Supervised (1\%) & 0.52 & 0.54 & 0.38 & 0.50  \\
         Ours (10\%) & 0.56 & 0.80 & 0.78 & 0.71  \\
         Ours (1\%) & 0.38 & 0.60 & 0.53 & 0.51  \\
         %\hline
         \hline
         Opaque Dataset & 0.02 & 0.04 & 0.06 & 0.03 \\

        %  Opaque Dataset & 0.42 & 0.31 & 0.24 & 0.32 \\
         %UW Pouring Dataset & - & - & - & -  \\
         \hline
    \end{tabular}
    \caption{Average Intersection over Union (IoU) scores on a test set of transparent liquid images, each filled with water to varying amounts.  We show the performance for subsets of images with varying amounts of liquid in the cup (Low, Medium, and High) as well as an average over all images. %The top group of methods are trained directly to perform on the evaluation domain. The bottom group of methods are trained on different liquids or different settings and evaluated on our test set.
    }
    \label{tab:vision}
\end{table}

\newcommand{\gridfig}[1]{\begin{subfigure}[t]{0.14\columnwidth}\includegraphics[width=\linewidth]{#1}\end{subfigure}}

\begin{figure}[ht!]
    \centering
    
    \begin{minipage}[t]{0.2\columnwidth}
        \textbf{Input}
    \end{minipage}
    \gridfig{images/results_figures/segmentation_visualizations/rgb_49.jpg}
    \gridfig{images/results_figures/segmentation_visualizations/rgb_63.jpg}
    \gridfig{images/results_figures/segmentation_visualizations/rgb_73.jpg}
    \gridfig{images/results_figures/segmentation_visualizations/rgb_85.jpg}
    \gridfig{images/results_figures/segmentation_visualizations/rgb_93.jpg}
    
    % \gridfig{images/results_figures/short/real_9.jpg}
    % \gridfig{images/results_figures/medium_1/real_22.jpg}
    % \gridfig{images/results_figures/medium_1/real_41.jpg}
    % \gridfig{images/results_figures/medium_2/real_37.jpg}
    % \gridfig{images/results_figures/tall/real_47.jpg}

    \par\smallskip
    
    \begin{minipage}[t]{0.20\columnwidth}
        \textbf{Ablation 1}
    \end{minipage}
    \gridfig{images/results_figures/segmentation_visualizations/rgb_49_ablation_1_maskThresholded.jpg}
    \gridfig{images/results_figures/segmentation_visualizations/rgb_63_ablation_1_maskThresholded.jpg}
    \gridfig{images/results_figures/segmentation_visualizations/rgb_73_ablation_1_maskThresholded.jpg}
    \gridfig{images/results_figures/segmentation_visualizations/rgb_85_ablation_1_maskThresholded.jpg}
    \gridfig{images/results_figures/segmentation_visualizations/rgb_93_ablation_1_maskThresholded.jpg}
    
    % \gridfig{images/results_figures/short/segmentation_9_ablation_2.jpg}
    % \gridfig{images/results_figures/medium_1/segmentation_22_ablation_2.jpg}
    % \gridfig{images/results_figures/medium_1/segmentation_41_ablation_2.jpg}
    % \gridfig{images/results_figures/medium_2/segmentation_37_ablation_2.jpg}
    % \gridfig{images/results_figures/tall/segmentation_47_ablation_2.jpg}
    
    \par\smallskip

    
    % \begin{minipage}[t]{0.20\columnwidth}
    %     \textbf{Ablation 2}
    % \end{minipage}
    % \gridfig{example-image-a}
    % \gridfig{example-image-a}
    % \gridfig{example-image-a}
    % \gridfig{example-image-a}
    % \gridfig{example-image-a}

    % \par\smallskip
    
    \begin{minipage}[t]{0.20\columnwidth}
        \textbf{Ours}
    \end{minipage}
    \gridfig{images/results_figures/segmentation_visualizations/rgb_49_our_method_maskThresholded.jpg}
    \gridfig{images/results_figures/segmentation_visualizations/rgb_63_our_method_maskThresholded.jpg}
    \gridfig{images/results_figures/segmentation_visualizations/rgb_73_our_method_maskThresholded.jpg}
    \gridfig{images/results_figures/segmentation_visualizations/rgb_85_our_method_maskThresholded.jpg}
    \gridfig{images/results_figures/segmentation_visualizations/rgb_93_our_method_maskThresholded.jpg}
    % \gridfig{images/results_figures/ablation_1_corrected/ablation_1_corrected_9.jpg}
    % \gridfig{images/results_figures/ablation_1_corrected/ablation_1_corrected_22.jpg}
    % \gridfig{images/results_figures/ablation_1_corrected/ablation_1_corrected_41.jpg}
    % \gridfig{images/results_figures/ablation_1_corrected/ablation_1_corrected_37.jpg}
    % \gridfig{images/results_figures/ablation_1_corrected/ablation_1_corrected_47.jpg}
    
    \caption{Representative segmentations of our method compared to a model trained on images of colored liquid with segmentation labels obtained through background subtraction (``Ablation 1''), which is unable to accurately segment the liquid. }
    \label{fig:segmentation_results}
\end{figure}

Our results for transparent liquid segmentation can be found in Table~\ref{tab:vision} as well as in Fig~\ref{fig:segmentation_results} (bottom row). Our method generally succeeds at segmenting the liquid pixels in the image, achieving high IoU scores across the test set. However, our method experiences a small drop in performance on images in which the cup is filled to a high level (i.e. right-most image in ``Ours'' in Figure \ref{fig:segmentation_results}). We hypothesize that such examples have regions of liquid that are distant from a liquid-cup or liquid-air boundary; thus these cases are harder to classify when there are no refractive patterns to indicate the presence of liquid.

% \begin{itemize}
%     \item Describe evaluation procedure.
%     \item Describe the baselines we're comparing against.
%     \item Describe the "unfair" baselines we're comparing against. Mostly just the pretrained models.
% \end{itemize}

\subsection{Pouring Performance}
\label{sec:pouring_perf}
\begin{table}[ht]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline 
        & \shortstack{Transparent Liquid \\ Ours (RMSE)} & \shortstack{Colored Liquid \\ Background Subtraction (RMSE)} \\
        %   & $0 \rightarrow 50\%$ & $0 \rightarrow 75\%$ & $25\% \rightarrow 75\%$ & All \\ 
        
        \hline
        $0\% \rightarrow 25\%$ & $1.00 \pm 0.43\%$ & $8.46 \pm 2.14\%$ \\
        $0\% \rightarrow 50\%$ & $0.82 \pm 0.67\%$ & $1.86 \pm 0.71\%$ \\
        $0\% \rightarrow 75\%$ & $1.18 \pm 0.74\%$ & $1.57 \pm 0.50\%$ \\
        $25\% \rightarrow 75\%$ & $0.75 \pm 0.49\%$ & $1.61 \pm 0.65\%$ \\
        \hline
        All & $0.94 \pm 0.61\%$ & $3.38 \pm 3.18\%$ \\
        \hline
    \end{tabular}
    \caption{Percent error of the pouring system on both transparent and colored liquids. For transparent liquid pouring, we use our learned segmentation model; for colored liquid pouring, we use background subtraction. Contrary to expectations, our system performs better with transparent segmentation than with colored segmentation. }
    \label{tab:pouring}
\end{table}

% \begin{table}[ht]
%     \centering
%     \begin{tabular}{|c|c|c|}
%         \hline 
%         & Ours (RMSE) & Oracle (RMSE)\\
%         %   & $0 \rightarrow 50\%$ & $0 \rightarrow 75\%$ & $25\% \rightarrow 75\%$ & All \\ 
        
%         \hline
%         $0\% \rightarrow 25\%$ & $0.14 \pm 0.06 \textrm{ cm} / 1.00\% $ & -\\%\pm 0.43\%$ & - \\
%         $0\% \rightarrow 50\%$ & $0.12 \pm 0.09 \textrm{ cm}/ 0.82\% $ & -\\%\pm 0.67\%$ & - \\
%         $0\% \rightarrow 75\%$ & $0.17 \pm 0.10 \textrm{ cm}/ 1.18\% $ & -\\%\pm 0.74\%$ & - \\
%         $25\% \rightarrow 75\%$ & $0.11 \pm 0.07 \textrm{ cm}/ 0.75\% $ & -\\%\pm 0.49\%$ & - \\
%         \hline
%         All & - & - \\
%         \hline
%     \end{tabular}
%     \caption{Caption \dave{This table is too messy and there are no units}\dave{Fix the caption}}
%     \label{tab:pouring}
% \end{table}

To assess the utility and effectiveness of transparent liquid segmentation in our real robotic pouring system, we conduct a series of pouring trials. We choose four different initial fill-levels and target fill-levels (see Table \ref{tab:pouring}), and conduct 20 pouring trials for each fill-level. We measure the level of liquid achieved upon the controller reaching the final \texttt{NotPouring} state, and report the average error across each fill-level, as well as across all trials.

We conduct two sets of trials: first with transparent water, using our transparent liquid segmentation system; second with green-colored water, using the background-subtraction method described in the supplementary materials. Given the high accuracy of background subtraction, we consider this second task to represent how the system would perform with near-perfect segmentation. We opted not to evaluate using segmentation methods with poor performance, due to the high risk of spilling liquid in the workspace. Results can be found in Table \ref{tab:pouring}.

In the case of pouring transparent liquids, we are able to achieve the desired ratio $l_{\mathrm{target}}$ with an average accuracy of 0.94\%, which corresponds to a roughly 0.13cm error on average. Surprisingly, in the case of colored liquid (where background subtraction yields high-fidelity segmentation), accuracy is worse, with an average error of 3.38\% or 0.47cm error. However, when observing the system, we noticed that the bounding box computation is sensitive to segmentations with splashing/sloshing: in these cases, the bounding box overestimates the amount of liquid in the cup, and terminates pouring earlier than it should. Segmentations from our model pick up less of this transient liquid, and thus outperform the ``ground-truth'' segmentation. With a more sophisticated postprocessing step and controller, these effects could potentially be mitigated. 

% \begin{itemize}
%     \item Describe the pouring evaluation procedure.
%     \item Describe the oracle approach.
%     \item Describe that we didn't want to compare against bad algos because they caused spilling.
%     \item Mention the performance.
% \end{itemize}

\subsection{Visual Translation}

\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.15\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/image_translation_figures/realA_4.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/image_translation_figures/realA_13.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/image_translation_figures/realA_25.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/image_translation_figures/realA_37.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/image_translation_figures/realA_46.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/image_translation_figures/realA_51.png}
    \end{subfigure}
    
    \par\smallskip % force a bit of vertical whitespace

    \begin{subfigure}[b]{0.15\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/image_translation_figures/fakeB_4.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/image_translation_figures/fakeB_13.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/image_translation_figures/fakeB_25.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/image_translation_figures/fakeB_37.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/image_translation_figures/fakeB_46.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/image_translation_figures/fakeB_51.png}
    \end{subfigure}
    \caption{Image translation from colored liquid to transparent liquid by our trained model; \textbf{Top Row:} Real world colored liquid images from $\mathcal{D}_{\mathrm{color}}$; \textbf{Bottom Row:} Generated transparent liquid images}
    \label{fig:visual_translation}
\end{figure}


% PUTTING THIS HERE TO FIT IT IN THE FINAL PAGE

\newcommand{\ablationfig}[1]{\begin{subfigure}[t]{0.3\columnwidth}\includegraphics[width=\linewidth]{#1}\end{subfigure}}

\begin{figure}[ht!]
    \centering
    
    \begin{subfigure}[b]{.45\columnwidth}
            % \includegraphics[width=\linewidth]{images/novel_cups.pdf}

            \includegraphics[width=\linewidth]{images/novel_cups_short.pdf}
            % \ablationfig{images/cup_shape_generalization/widecup/widecup_short_blended_20.jpg} 
            % \ablationfig{images/cup_shape_generalization/widecup/widecup_medium_blended_17.jpg} 
            % \ablationfig{images/cup_shape_generalization/widecup/widecup_tall_blended_15.jpg}
            
            % \par\smallskip
            
            % \ablationfig{images/cup_shape_generalization/square_cup/square_cup_short_blended_33.jpg} 
            % \ablationfig{images/cup_shape_generalization/square_cup/square_cup_medium_blended_29.jpg} 
            % \ablationfig{images/cup_shape_generalization/square_cup/square_cup_tall_blended_5.jpg}

            % \par\smallskip

            % \ablationfig{images/cup_shape_generalization/sphere_jar/sphere_jar_short_blended_45.jpg} 
            % \ablationfig{images/cup_shape_generalization/sphere_jar/sphere_jar_medium_blended_41.jpg} 
            % \ablationfig{images/cup_shape_generalization/sphere_jar/sphere_jar_tall_blended_17.jpg}

            % \par\smallskip


            % \ablationfig{images/cup_shape_generalization/tallcup/tallcup_short_blended_9.jpg} 
            % \ablationfig{images/cup_shape_generalization/tallcup/tallcup_medium_blended_6.jpg} 
            % \ablationfig{images/cup_shape_generalization/tallcup/tallcup_tall_blended_0.jpg}
            
            % \par\smallskip
            
            % \ablationfig{images/cup_shape_generalization/conecup/conecup_short_blended_64.jpg} 
            % \ablationfig{images/cup_shape_generalization/conecup/conecup_medium_blended_62.jpg}
            % \ablationfig{images/cup_shape_generalization/conecup/conecup_tall_blended_56.jpg}
            
            % \par\smallskip
            
            % \ablationfig{images/cup_shape_generalization/nescafe_jar/nescafe_jar_short_blended_128.jpg} 
            % \ablationfig{images/cup_shape_generalization/nescafe_jar/nescafe_jar_medium_blended_117.jpg} 
            % \ablationfig{images/cup_shape_generalization/nescafe_jar/nescafe_jar_tall_blended_102.jpg}

        \caption{}
        \label{fig:novel_cups}

    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.45\columnwidth}
          \ablationfig{images/diverse_background_generalization/short/blended_1.jpg}
          \ablationfig{images/diverse_background_generalization/medium/blended_38.jpg}
          \ablationfig{images/diverse_background_generalization/tall/blended_4.jpg}
          
          \par\smallskip

          
          \ablationfig{images/diverse_background_generalization/short/blended_6.jpg}
          \ablationfig{images/diverse_background_generalization/medium/blended_39.jpg}
          \ablationfig{images/diverse_background_generalization/tall/blended_43.jpg}
          
          \par\smallskip

             
          \ablationfig{images/diverse_background_generalization/short/blended_42.jpg}
          \ablationfig{images/diverse_background_generalization/medium/blended_89.jpg}
          \ablationfig{images/diverse_background_generalization/tall/blended_424.jpg}
          
          \par\smallskip

            
        % Removing examples from the figure for space reasons.
        %   \ablationfig{images/diverse_background_generalization/short/blended_103.jpg}
        %   \ablationfig{images/diverse_background_generalization/medium/blended_97.jpg}
        %   \ablationfig{images/diverse_background_generalization/tall/blended_337.jpg}
           
        %   \par\smallskip

           
        %   \ablationfig{images/diverse_background_generalization/short/blended_484.jpg}
        %   \ablationfig{images/diverse_background_generalization/medium/blended_474.jpg}
        %   \ablationfig{images/diverse_background_generalization/tall/blended_454.jpg}
          
        \caption{}
          \label{fig:novel_backgrounds}

    \end{subfigure}
    
    
    \caption{Generalization of our transparent liquid segmentation model. In (a), we show that when our segmentation model is trained on one specific kind of cup in a scene (top row), it is able to generalize reasonably to unseen transparent cups in the same scene. In (b), we show that when our segmentation model is trained on a diverse set of background images, it is able to effectively generalize to novel backgrounds.}
    \label{fig:generalization}
\end{figure}


	We show representative examples of the image translation achieved by our CUT-based model in Fig~\ref{fig:visual_translation}. We observe that the network is able to translate the input image containing green-colored water pixels into images of clear water while still capturing the same background and refraction patterns as that in the source image. Most importantly, the transparent liquid in the synthetic images is in the same location as the colored liquid in the original images. This property allows us to apply the background mask from the colored liquids as the ground-truth label for the synthetic images of transparent liquids.

\subsection{Visual Ablations}

\noindent \textbf{Ablation 1: What is the benefit of training the segmentation model on synthetically generated transparent (instead of colored) liquid?} To answer this question, we train a segmentation model on colored liquid with color jitter and evaluate it on transparent liquid. We jitter the brightness, contrast and hue to obtain the input image for training the segmentation model. This ablation explores whether such color augmentation is sufficient to train a model for transparent liquid segmentation. 
% , compared to our method (``Ours"). The average IoU of 0.32 shows that the segmentation model trained from scratch is mostly to unable classify liquid vs non-liquid pixels.
Quantitative results of this ablation (``Opaque Dataset'') are shown in Table~\ref{tab:vision}. Qualitative results are shown in Fig~\ref{fig:segmentation_results}. The model fails to detect the correct liquid height during our evaluation. This analysis shows that using color jitter on a colored liquid image is not sufficient domain randomization to capture the texture and patterns required to segment transparent liquids, supporting the idea that the segmentation model should be trained directly on images of transparent liquid.

\par\smallskip

\noindent \textbf{Ablation 2: What is the benefit of the translation approach over using a small amount of manually-labeled data?} Since our method uses a standard supervised loss function to train the model on synthetic data, a natural comparison is to evaluate performance when the model is trained on images of transparent images with manual segmentation annotations. Since annotation is very time-consuming ($\sim$1min per image), we annotate 10\% of images in the training domain, and observe how well the model can learn to segment on two supervised subsets: 10\% labeled and 1\% labeled. Additionally, we train our method on same fraction of images from our synthetic dataset. Results can be found in the second section of Table \ref{tab:vision}.

We draw two conclusions from these results. First, both our method and the fully-supervised ablation require substantially less data to reach their peak performance on the test set than is available: ``Ours (10\%)'' shows the same performance as our full method (``Ours''), and ``Supervised (10\%)'' outperforms our method. This is unsurprising, given that our test images are visually quite similar to the training set. Second, with only 1\% of manually-annotated labels available, the supervised baseline (``Supervised (1\%)'') performs substantially worse than our full method. While our dataset is rather small -- we were able to manually label 10\% of the data -- our data collection method is extremely scalable. In large datasets it is reasonable to expect one might only have access to manually-annotated labels for 1\% of a full dataset. This provides evidence that our method would scale well to liquid datasets where a small amount of supervised data would not provide sufficient generalization.

\par\smallskip

% \noindent \textbf{Ablation 3: What is the benefit of using this approach instead of transferring a model from a large existing dataset?} \ben{write this when we have results}

% \par\smallskip



\noindent \textbf{Ablation 3: Does the approach work if there are diverse cups and backgrounds?} To evaluate our segmentation model's capacity to generalize to diverse cups and backgrounds, we conduct two studies, shown in Figure \ref{fig:generalization}. We first train a segmentation model on an image dataset consisting of a single cup in a single scene with varying heights of liquids. We then evaluate on transparent cups of different shapes with different fill levels of transparent liquid. As can be seen in Figure \ref{fig:novel_cups}, the model generalizes reasonably to other cups, indicating that it has learned to detect relevant liquid features invariant a specific container. Next, we train a model on a cup in front of a diverse set of backgrounds and various water heights, with a dataset collected as described in Section \ref{sec:backgrounds}. As can be seen in Figure \ref{fig:novel_backgrounds}, the model learns a segmentation function that is invariant to novel unseen backgrounds. These two experiments demonstrate the potential of our approach to scale to a general set of scenes, provided a sufficiently diverse dataset generated by our method.










